Turnpike properties in nonlinear system identification

We analyze the problem of learning general discrete-time nonlinear state-space models using the simulation error minimization (SEM) method. In this setting, model parameters are typically learned by minimizing the mismatch between simulated and measured outputs over a training dataset, or shorter subsequences extracted from it. Specifically, we study the cumulative output turnpike property of the underlying SEM optimization problem, which requires optimal output sequences emanating from a fixed initial state to approach and remain close to an optimal output sequence of the corresponding SEM problem with free initial state. In the presence of non-unique optimal output sequences---as may arise, for instance, in fully black-box system identification using neural networks---the property is formulated with respect to the closest such sequence. Turnpike behavior is generally desirable in practice, as it provides a theoretical justification for employing computationally more tractable SEM formulations with fixed initial states while ensuring that their optimal output sequences remain close to unconstrained optimal ones. Under a mild reachability condition, we establish equivalence between the cumulative turnpike property, coercivity of the value function, and a tailored notion of strict dissipativity. We additionally introduce a cardinality turnpike property and show that it is strictly weaker than the cumulative notion. Finally, we establish sufficient conditions for turnpike behavior based on incremental output stability, convexity of the stage cost, and a suitable optimality condition, and illustrate the theory by means of a numerical example.

==> numerical_example_1.tex <==
\section{Example}\label{sec:example}

To illustrate the theory presented, we deliberately consider a simplified setting: the identification of a scalar linear state-space model. This allows us to study solutions to the SEM problem analytically and, where needed, using standard numerical optimization methods. For larger benchmark examples illustrating in particular the role of a burn-in phase in recurrent neural network training using the SEM method, the reader is referred to~\cite{Schiller2025b}.
Here, we consider the model%
\begin{equation}
	x^+ = \theta x + u, \qquad y=x, \label{eq:ex_sys}
\end{equation}
where $\theta$ is the parameter be identified.
To this end, we generate a (noisy) training dataset $D$ as in~\eqref{eq:Di} by simulating the model~\eqref{eq:ex_sys} using the true unknown parameter $\theta^\mathrm{true} = 0.8$, initial condition $x_0^\mathrm{true}=-2$, and a sinusoidal input trajectory $U^\mathrm{d}$; the output measurements $y^\mathrm{d}_j$ are corrupted by additional normally distributed measurement noise.
In our experiments, $D$ satisfies $(u_j^\mathrm{d},y_j^\mathrm{d})\in\mathcal{U}^\mathrm{d}\times\mathcal{Y}^\mathrm{d}$, $j\in[0,N]$, with $\mathcal{U}^\mathrm{d}=\mathcal{Y}^\mathrm{d}=[-c_\mathrm{d},c_\mathrm{d}]$ and $c_\mathrm{d}=2$.
Moreover, we consider the sets $\mathcal{X}_0 = [-c_\mathrm{x},c_\mathrm{x}]$ and $\Theta = [-c_\theta,c_\theta]$ with $c_\mathrm{x}=10$ and $c_\theta=0.9$, respectively.
Given some $(x_0,\theta)$ and the input sequence $U^\mathrm{d}$, the model~\eqref{eq:ex_sys} produces the outputs
\begin{equation}
	y_j=y_j(x_0,\theta,U^\mathrm{d}) = \theta^jx_0+ \sum_{t=0}^{j-1}\theta^{j-t-1}u_t^\mathrm{d},\  \ j\in[0{,}N]. \label{eq:ex_dyn}
\end{equation}
As $\mathcal{X}_0$, $\Theta$, and $\mathcal{U}^\mathrm{d}$ are bounded, there exists a compact set $\mathcal{Y}\subset\mathbb{R}$ such that $y_j\in\mathcal{Y}$ for all $j\in[0,N]$ and all $N\in\mathbb{N}$.
%$y_j\in\mathcal{Y}$ for all $j\in[0,N]$ uniformly in $N$ with $\mathcal{Y}=\{y\in\mathbb{R} \mid |y|\leq c_x + c_\mathrm{d}/(1-c_\theta)\}$ using~\eqref{eq:ex_dyn}, the triangle inequality, and boundedness of $\mathcal{X}_0$, $\Theta$, and $\mathcal{U}^\mathrm{d}$.

We aim to identify the unknown parameter $\theta$ using the constrained SEM problem~\eqref{eq:NLP_case_1}. To this end, we set $\bar{x} = 1$ and consider the cost function in~\eqref{eq:NLP_cost} with $l(y_1,y_2) = (y_1 - y_2)^2$ and $r \equiv 0$, including a burn-in phase of length $m = 10$ (cf. Section~\ref{sec:coerc}) and varying data sizes $N \in \mathbb{N}$ with $N \geq m$.

\begin{claim}\label{claim}
	The value function~\eqref{eq:NLP_case_1} is coercive (Definition~\ref{def:coerc}). The output turnpike is cheaply reachable (Assumption~\ref{ass:reachability}).
\end{claim}

The first statement directly follows by application of Theorem~\ref{thm:coerc}; indeed, the model~\eqref{eq:ex_sys} is linear and stable, $\mathcal{Y}$ is compact, and $l$ is strictly convex, so that Assumption~\ref{ass:convex_lr} holds with $\phi(s)=\frac{\kappa}{2} s^2$, $\kappa>0$, and Assumption~\ref{ass:optimality} holds with some $K>0$.
\red{NO: maybe consider noise-free data, giving $V^*=0$; or	bounded finite-energy noise, maybe decaying far in the future...}
For the second statement, note that $l$ satisfies Assumption~\ref{ass:Lipschitz} and, using~\eqref{eq:ex_dyn}, the triangle inequality, and boundedness of $\mathcal{X}_0$ and $\Theta$, one verifies~\eqref{eq:output_stability}, i.e., Assumption~\ref{ass:output_stability}, with $\lambda = c_\theta$ and $C = 1$. Hence, the conditions of Proposition~\ref{prop:reachability} are satisfied, and Assumption~\ref{ass:reachability} holds.

%First, we note that $l$ is locally Lipschitz continuous in the sense of Assumption~\ref{ass:Lipschitz}), where a possible Lipschitz constant $L$ can be computed using compactness of $\mathcal{Y},\mathcal{Y}^\mathrm{d}$, leading to $L= 2(c_x+2/(1-c_\theta)+2)$.
%\begin{equation*}
%	L=2\left(\max_{y\in\mathcal{Y}}\|y\| + \max_{y\in\mathcal{Y}^\mathrm{d}}\|y\|\right) = c_x+2/(1-c_\theta)+2.
%\end{equation*}
%Moreover, using~\eqref{eq:ex_dyn} and the triangle inequality, we can obtain that $\|y_j(x_0,\theta,U^\mathrm{d})-y_j(\bar{x}_0,\theta,U^\mathrm{d})\| \leq c_\theta^j\|x_0-\bar{x}_0\|$, $j\in[0,N]$ for all $x_0,\bar{x}_0\in\mathcal{X}_0$ uniformly and all $\theta\in\Theta$, which verifies Assumption~\ref{ass:output_stability} with $\lambda=c_\theta$ and $C=1$.
%Consequently, all conditions of Proposition~\ref{prop:reachability} are satisfied, and Assumption~\ref{ass:reachability} holds for $E_\mathrm{r} = {2c_xL}/(1-c_\theta)<\infty$.

\emph{Consequently, by application of Theorem~\ref{thm:equivalences}, the SEM identification problem in~\eqref{eq:NLP_case_1} is strictly dissipative (Definition~\ref{def:diss}) and has the cumulative turnpike property (Definition~\ref{def:intTP}).}

Let us now consider $N=m$. Then, the cost function reduces to $J(x_0,\theta) = (y_N(x_0,\theta,U^\mathrm{d}) - y_N^\mathrm{d})^2$, where we assume that $y_N^\mathrm{d}\neq 0$. 
This corresponds to learning a one-step predictor after processing the full input sequence $U^\mathrm{d}$, which is of practical relevance, e.g., in time series forecasting; see \cite{Hewamalage2021}. Hence, it follows that $V^* = 0$, which is attained whenever $y_N(x_0,\theta,U^\mathrm{d}) = y_N^\mathrm{d}$, that is, for any pair $(x_0,\theta)$ with $\theta \neq 0$ satisfying
\begin{equation}\label{eq:ex_thetax0}
	x_0 = \frac{y^\mathrm{d}_N-\sum_{j=0}^{N-1}\theta^{N-j-1}u_j^\mathrm{d}}{\theta^N}.
\end{equation}
This describes a curve in the $\theta x_0$-plane, depicted by the blue line in the middle plot of Figure~\ref{fig:example}.
The solution set $\mathcal{S}^*$ in~\eqref{eq:S_star} corresponds to the admissible part of this curve, that is, $\mathcal{S}^* = \left\{(x_0,\theta)\in\mathcal{X}_0\times\Theta \mid \eqref{eq:ex_thetax0}, \theta\neq 0 \right\}$; see the red (solid/dotted) lines in the middle plot of Figure~\ref{fig:example}.
Using~\eqref{eq:ex_dyn} and~\eqref{eq:ex_thetax0}, the optimal output at time $j\in[0,N]$ can be expressed as a function of $\theta\in\Theta$ as $y_j(x_0^*,\theta^*,U^\mathrm{d}) = \theta^{j-N}y^\mathrm{d}_N-\sum_{k=j}^{N-1}\theta^{j-k-1}u_k^\mathrm{d}$.
Since $y_N(x_0^*,\theta^*,U^\mathrm{d}) = y^\mathrm{d}_N$ for all $(x_0^*,\theta^*)\in\mathcal{S}^*$, the set $\mathcal{S}^*(x_0,\theta)$ defined in~\eqref{eq:set_S0x} is independent of $(x_0,\theta)$, leading to $\mathcal{S}^*(x_0,\theta) = \mathcal{S}^*$.

%\begin{align*}
%	\mathcal{S}^*(x_0,\theta) &= \left\{ \arg\min_{(x_0',\theta')\in\mathcal{S}^*} \left(y^\mathrm{d}_N - \theta^Nx_0 - \sum_{j=0}^{N-1}\theta^{t-j-1}u_j^\mathrm{d}\right)^2\right\}\\
%	&= \mathcal{S}^*
%\end{align*}



We now consider the constrained SEM problem in~\eqref{eq:NLP_case_1}. The left plot in Figure~\ref{fig:example} depicts the cost function $J(\bar{x},\theta)$ as a function of $\theta$, from which it follows that $\mathcal{S}'(\bar{x}) = \{\theta'\}$ with $\theta' = -0.65$.
Thus, the properties in Definitions~\ref{def:intTP}--\ref{def:cardTP} hold for the pair $(\bar{x},\theta')$ uniformly for all $(x_0^*,\theta^*)\in\mathcal{S}^*$. The right plot in Figure~\ref{fig:example} (red regions) shows the family of output differences associated with all $(x_0^*,\theta^*)\in\mathcal{S}^*$; these sequences converge to a common value, illustrating the turnpike behavior and its independence of $(x_0^*,\theta^*)$.

To further illustrate the turnpike property, we additionally consider $N\in 2\cdot\{10^1, 10^2, 10^3, 10^4\}$, where we solve the SEM problems in \eqref{eq:NLP_case_TP} and~\eqref{eq:NLP_case_1} in MATLAB using the \texttt{fmincon}-routine. The corresponding solutions are found to be unique, leading to $\mathcal{S}^* = \{(x_0^*,\theta^*)\}$ and $\mathcal{S}'(\bar{x}) = \{\theta'\}$, as indicated in the middle plot of Figure~\ref{fig:example}. The right plot shows that, as $N$ increases, the corresponding output sequences become progressively closer to each other. This behavior is consistent with the theory and illustrates the cumulative turnpike property in Definition~\ref{def:intTP}.



\begin{figure*}
	\vspace{1.2ex}
	\includegraphics{ex_Jprime_mod}\hfill
	\includegraphics{ex_theta_x0_mod}\hfill
	\includegraphics{ex_f_ey}
	\caption{Left: Cost function $J(\bar{x},\theta)$ over $\theta\in\Theta$ for $N=m=10$. Middle: Solution sets $\mathcal{S}^*$ (solid/dotted red line, $\times$-markers) and $\mathcal{S}'(\bar{x})$ (dot-markers) in the $\theta x_0$-plane for different values of $N$ (the colors coincide with the legend of the right plot). Right: Squared output differences over times $j\in[0,N]$.}
	\label{fig:example}
\end{figure*}

